A Survey of Approaches for Event Sequence Analysis and Visualization using the ESeVis Framework

Event sequence data is increasingly available. Many business operations are supported by information systems that record transactions, events, state changes, message exchanges, and so forth. This observation is equally valid for various industries, including production, logistics, healthcare, financial services, education, to name but a few. The variety of application areas explains that techniques for event sequence data analysis have been developed rather independently in different fields of computer science. Most prominent are contributions from information visualization and from process mining. So far, the contributions from these two fields have neither been compared nor have they been mapped to an integrated framework. In this paper, we develop the Event Sequence Visualization framework (ESeVis) that gives due credit to the traditions of both fields. Our mapping study provides an integrated perspective on both fields and identifies potential for synergies for future research.

==> tables/1-BPI2018-example.tex <==
\begin{tabular}{l r r r r}
	\toprule
	%\textbf{Approach} &  \multicolumn{5}{c}{\textbf{Requirements}}  \\
	%\cmidrule{2-6} & \textbf{R1} & \textbf{R2}& \textbf{R3} & \textbf{R4} & \textbf{R5} \\
%	\textbf{Step} & 1 & 2 & 3 & 4 & 5 \\
	\textbf{activity} & calculate & decide & begin payment & abort payment \\
	\textbf{resource} & 727350 & 8beb64 & DP-Z & DP-Z \\
	\textbf{subprocess} & Application & Application & Application & Application  \\
	\textbf{timestamp} & 2015-12-04T22:27:42 & 2015-12-05T10:57:48 & 2015-12-17T08:48:14 & 2015-12-18T12:41:18  \\
	\textbf{identity:id} & 00D38D7C-5FDE... & 5C2FAF2F-5D77... & 825324F8-DFD2... & B8A341A0-429F...  \\
	\textbf{docid} & -900661955861908 & -1080805941013282 & -180086114957438 & -180086114957438   \\
	\textbf{success} & true & true	 & true & true  \\
	\textbf{note} & automatic & automatic & automatic during payment & automatic during payment \\
	\midrule
	\textbf{application (Case)} & \multicolumn{4}{c}{a5d4750c95b54685}  \\
	\textbf{young farmer} & \multicolumn{4}{c}{false}   \\		
	\textbf{number parcels} & \multicolumn{4}{c}{4}  \\		
	\textbf{amount applied} & \multicolumn{4}{c}{2002.6} \\
	\bottomrule
\end{tabular}

%<event>
%	<boolean key="success" value="true"/>
%	<string key="org:resource" value="727350"/>
%	<id key="docid_uuid" value="82F4E3D1-E9C9-41E2-93E0-4AD7B57410FF"/>
%	<string key="doctype" value="Payment application"/>
%	<string key="subprocess" value="Application"/>
%	<string key="docid" value="-18008611495743853"/>
%	<string key="activity" value="calculate"/>
%	<string key="note" value="automatic"/>
%	<string key="eventid" value="-90066195586190856"/>
%	<id key="identity:id" value="00D38D7C-5FDE-4A10-B04E-A975A1AB09DD"/>
%	<string key="concept:name" value="calculate"/>
%	<string key="lifecycle:transition" value="complete"/>
%	<date key="time:timestamp" value="2015-12-04T22:27:42.704+01:00"/>
%</event>

%<event>
%	<boolean key="success" value="true"/>
%	<string key="org:resource" value="8beb64"/>
%	<id key="docid_uuid" value="82F4E3D1-E9C9-41E2-93E0-4AD7B57410FF"/>
%	<string key="doctype" value="Payment application"/>
%	<string key="subprocess" value="Application"/>
%	<string key="docid" value="-18008611495743853"/>
%	<string key="activity" value="decide"/>
%	<string key="note" value="automatic"/>
%	<string key="eventid" value="-108080594101328239"/>
%	<id key="identity:id" value="5C2FAF2F-5D77-4B2E-BFD4-CCF01F438A8F"/>
%	<string key="concept:name" value="decide"/>
%	<string key="lifecycle:transition" value="complete"/>
%	<date key="time:timestamp" value="2015-12-05T10:57:48.254+01:00"/>
%</event>
%<event>
%	<boolean key="success" value="true"/>
%	<string key="org:resource" value="DP-Z"/>
%	<id key="docid_uuid" value="82F4E3D1-E9C9-41E2-93E0-4AD7B57410FF"/>
%	<string key="doctype" value="Payment application"/>
%	<string key="subprocess" value="Application"/>
%	<string key="docid" value="-18008611495743853"/>
%	<string key="activity" value="begin payment"/>
%	<string key="note" value="automatic during payment"/>
%	<string key="eventid" value="-18008597326795840"/>
%	<id key="identity:id" value="825324F8-DFD2-4B8E-8A17-B5CF02544ED0"/>
%	<string key="concept:name" value="begin payment"/>
%	<string key="lifecycle:transition" value="complete"/>
%	<date key="time:timestamp" value="2015-12-17T08:48:14.861+01:00"/>
%</event>
%<event>
%	<boolean key="success" value="true"/>
%	<string key="org:resource" value="DP-Z"/>
%	<id key="docid_uuid" value="82F4E3D1-E9C9-41E2-93E0-4AD7B57410FF"/>
%	<string key="doctype" value="Payment application"/>
%	<string key="subprocess" value="Application"/>
%	<string key="docid" value="-18008611495743853"/>
%	<string key="activity" value="abort payment"/>
%	<string key="note" value="automatic during payment"/>
%	<string key="eventid" value="-18008596977165086"/>
%	<id key="identity:id" value="B8A341A0-429F-4A2A-BB4B-280DA44902F1"/>
%	<string key="concept:name" value="abort payment"/>
%	<string key="lifecycle:transition" value="complete"/>
%	<date key="time:timestamp" value="2015-12-18T12:41:18.130+01:00"/>
%</event>
%<event>
%	<boolean key="success" value="true"/>
%	<string key="org:resource" value="DP-Z"/>
%	<id key="docid_uuid" value="82F4E3D1-E9C9-41E2-93E0-4AD7B57410FF"/>
%	<string key="doctype" value="Payment application"/>
%	<string key="subprocess" value="Application"/>
%	<string key="docid" value="-18008611495743853"/>
%	<string key="activity" value="begin payment"/>
%	<string key="note" value="automatic during payment"/>
%	<string key="eventid" value="-18008596507544968"/>
%	<id key="identity:id" value="67445AA3-557F-4457-A42F-46585563D00D"/>
%	<string key="concept:name" value="begin payment"/>
%	<string key="lifecycle:transition" value="complete"/>
%	<date key="time:timestamp" value="2015-12-19T06:10:14.446+01:00"/>
%</event>
%<event>
%	<boolean key="success" value="true"/>
%	<string key="org:resource" value="DP-Z"/>
%	<id key="docid_uuid" value="82F4E3D1-E9C9-41E2-93E0-4AD7B57410FF"/>
%	<string key="doctype" value="Payment application"/>
%	<string key="subprocess" value="Application"/>
%	<string key="docid" value="-18008611495743853"/>
%	<string key="activity" value="finish payment"/>
%	<string key="note" value="automatic during payment"/>
%	<string key="eventid" value="-18008575555842716"/>
%	<id key="identity:id" value="EAB9E552-F563-4221-BA8A-D0FAAEF94F19"/>
%	<string key="concept:name" value="finish payment"/>
%	<string key="lifecycle:transition" value="complete"/>
%	<date key="time:timestamp" value="2016-02-18T07:28:21.194+01:00"/>
%</event>
%%
%
%<trace>
%<boolean key="young farmer" value="false"/>
%<boolean key="selected_random" value="false"/>
%<boolean key="penalty_AJLP" value="false"/>
%<string key="application" value="a5d4750c95b54685"/>
%<float key="penalty_amount0" value="0.0"/>
%<string key="program-id" value="215"/>
%<boolean key="penalty_BGKV" value="false"/>
%<boolean key="penalty_AUVP" value="false"/>
%<string key="applicant" value="4f7db06718ede1bf"/>
%<float key="risk_factor" value="1.0"/>
%<boolean key="small farmer" value="false"/>
%<boolean key="penalty_BGP" value="false"/>
%<string key="department" value="4e"/>
%<boolean key="penalty_C16" value="false"/>
%<boolean key="penalty_BGK" value="false"/>
%<boolean key="penalty_AVUVP" value="false"/>
%<boolean key="penalty_CC" value="false"/>
%<boolean key="penalty_AVJLP" value="false"/>
%<boolean key="penalty_C9" value="false"/>
%<float key="cross_compliance" value="0.0"/>
%<boolean key="rejected" value="false"/>
%<boolean key="greening" value="true"/>
%<boolean key="penalty_C4" value="false"/>
%<boolean key="penalty_AVGP" value="false"/>
%<boolean key="penalty_ABP" value="false"/>
%<boolean key="penalty_B6" value="false"/>
%<boolean key="penalty_B4" value="false"/>
%<boolean key="penalty_B5" value="false"/>
%<boolean key="penalty_AVBP" value="false"/>
%<boolean key="penalty_B2" value="false"/>
%<boolean key="selected_risk" value="false"/>
%<boolean key="penalty_B3" value="false"/>
%<float key="area" value="5.8306"/>
%<boolean key="selected_manually" value="false"/>
%<boolean key="penalty_AGP" value="false"/>
%<boolean key="penalty_B16" value="false"/>
%<boolean key="penalty_GP1" value="false"/>
%<boolean key="basic payment" value="true"/>
%<boolean key="penalty_B5F" value="false"/>
%<boolean key="penalty_V5" value="false"/>
%<float key="payment_actual0" value="2002.6"/>
%<id key="identity:id" value="7D8833EE-2F8C-44C4-8391-A5D5473B0B57"/>
%<float key="amount_applied0" value="2002.6"/>
%<boolean key="redistribution" value="true"/>
%<boolean key="penalty_JLP6" value="false"/>
%<boolean key="penalty_JLP7" value="false"/>
%<string key="year" value="2015"/>
%<boolean key="penalty_JLP5" value="false"/>
%<boolean key="penalty_JLP2" value="false"/>
%<boolean key="penalty_JLP3" value="false"/>
%<int key="number_parcels" value="4"/>
%<boolean key="penalty_JLP1" value="false"/>
%<string key="concept:name" value="a5d4750c95b54685"/>

